Value Function Based Performance Optimization of Deep Learning Workloads

As machine learning techniques become ubiquitous, the efficiency of neural network implementations is becoming correspondingly paramount. Frameworks, such as Halide and TVM, separate out the algorithmic representation of the network from the schedule that determines its implementation. Finding good schedules, however, remains extremely challenging. We model this scheduling problem as a sequence of optimization choices, and present a new technique to accurately predict the expected performance of a partial schedule. By leveraging these predictions we can make these optimization decisions greedily and rapidly identify an efficient schedule. This enables us to find schedules that improve the throughput of deep neural networks by 2.6x over Halide and 1.5x over TVM. Moreover, our technique is two to three orders of magnitude faster than that of these tools, and completes in seconds instead of hours.

==> 12-references.tex <==

@misc{TF,
title={ {TensorFlow}: Large-Scale Machine Learning on Heterogeneous Systems},
url={https://www.tensorflow.org/},
note={Software available from tensorflow.org},
author={
    Mart\'{\i}n~Abadi and
    Ashish~Agarwal and
    Paul~Barham and
    Eugene~Brevdo and
    Zhifeng~Chen and
    Craig~Citro and
    Greg~S.~Corrado and
    Andy~Davis and
    Jeffrey~Dean and
    Matthieu~Devin and
    Sanjay~Ghemawat and
    Ian~Goodfellow and
    Andrew~Harp and
    Geoffrey~Irving and
    Michael~Isard and
    Yangqing Jia and
    Rafal~Jozefowicz and
    Lukasz~Kaiser and
    Manjunath~Kudlur and
    Josh~Levenberg and
    Dandelion~Man\'{e} and
    Rajat~Monga and
    Sherry~Moore and
    Derek~Murray and
    Chris~Olah and
    Mike~Schuster and
    Jonathon~Shlens and
    Benoit~Steiner and
    Ilya~Sutskever and
    Kunal~Talwar and
    Paul~Tucker and
    Vincent~Vanhoucke and
    Vijay~Vasudevan and
    Fernanda~Vi\'{e}gas and
    Oriol~Vinyals and
    Pete~Warden and
    Martin~Wattenberg and
    Martin~Wicke and
    Yuan~Yu and
    Xiaoqiang~Zheng},
  year={2015},
}




@article{halide_autoschedule,
 author = {Adams, Andrew and Ma, Karima and Anderson, Luke and Baghdadi, Riyadh and Li, Tzu-Mao and Gharbi, Micha\"{e}l and Steiner, Benoit and Johnson, Steven and Fatahalian, Kayvon and Durand, Fr{\'e}do and Ragan-Kelley, Jonathan},
 title = {Learning to Optimize Halide with Tree Search and Random Programs},
 journal = {ACM Trans. Graph.},
 issue_date = {July 2019},
 volume = {38},
 number = {4},
 month = jul,
 year = {2019},
 issn = {0730-0301},
 pages = {121:1--121:12},
 articleno = {121},
 numpages = {12},
 url = {http://doi.acm.org/10.1145/3306346.3322967},
 doi = {10.1145/3306346.3322967},
 acmid = {3322967},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {halide, optimizing compilers},
} 

@inproceedings {tvm_compiler,
author = {Tianqi Chen and Thierry Moreau and Ziheng Jiang and Lianmin Zheng and Eddie Yan and Haichen Shen and Meghan Cowan and Leyuan Wang and Yuwei Hu and Luis Ceze and Carlos Guestrin and Arvind Krishnamurthy},
title = {{TVM}: An Automated End-to-End Optimizing Compiler for Deep Learning},
booktitle = {13th {USENIX} Symposium on Operating Systems Design and Implementation ({OSDI} 18)},
year = {2018},
isbn = {978-1-939133-08-3},
address = {Carlsbad, CA},
pages = {578--594},
url = {https://www.usenix.org/conference/osdi18/presentation/chen},
publisher = {{USENIX} Association},
month = oct,
}

@inproceedings{tvm,
 author = {Chen, Tianqi and Zheng, Lianmin and Yan, Eddie and Jiang, Ziheng and Moreau, Thierry and Ceze, Luis and Guestrin, Carlos and Krishnamurthy, Arvind},
 title = {Learning to Optimize Tensor Programs},
 booktitle = {Proceedings of the 32Nd International Conference on Neural Information Processing Systems},
 series = {NIPS'18},
 year = {2018},
 location = {Montr\&\#233;al, Canada},
 pages = {3393--3404},
 numpages = {12},
 url = {http://dl.acm.org/citation.cfm?id=3327144.3327258},
 acmid = {3327258},
 publisher = {Curran Associates Inc.},
 address = {USA},
} 


@article{halide,
author = {Ragan-Kelley, Jonathan and Adams, Andrew and Paris, Sylvain and Levoy, Marc and Amarasinghe, Saman and Durand, Frédo},
year = {2012},
month = {07},
pages = {},
title = {Decoupling Algorithms from Schedules for Easy Optimization of Image Processing Pipelines},
volume = {31},
journal = {ACM Transactions on Graphics - TOG},
doi = {10.1145/2185520.2185528}
}

@article{old_halide_scheduler,
 author = {Mullapudi, Ravi Teja and Adams, Andrew and Sharlet, Dillon and Ragan-Kelley, Jonathan and Fatahalian, Kayvon},
 title = {Automatically Scheduling Halide Image Processing Pipelines},
 journal = {ACM Trans. Graph.},
 issue_date = {July 2016},
 volume = {35},
 number = {4},
 month = jul,
 year = {2016},
 issn = {0730-0301},
 pages = {83:1--83:11},
 articleno = {83},
 numpages = {11},
 url = {http://doi.acm.org/10.1145/2897824.2925952},
 doi = {10.1145/2897824.2925952},
 acmid = {2925952},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {halide, image processing, optimizing compilers},
} 


@inproceedings{mullapudi,
  title={Automatically scheduling halide image processing pipelines},
  author={Ravi Teja Mullapudi and Andrew Adams and Dillon Sharlet and Jonathan Ragan-Kelley and and Kayvon Fatahalia},
  booktitle={ACM Trans. Graph},
  year={2016},
}


@incollection{pytorch,
title = {PyTorch: An Imperative Style, High-Performance Deep Learning Library},
author = {Paszke, Adam and Gross, Sam and Massa, Francisco and Lerer, Adam and Bradbury, James and Chanan, Gregory and Killeen, Trevor and Lin, Zeming and Gimelshein, Natalia and Antiga, Luca and Desmaison, Alban and Kopf, Andreas and Yang, Edward and DeVito, Zachary and Raison, Martin and Tejani, Alykhan and Chilamkurthy, Sasank and Steiner, Benoit and Fang, Lu and Bai, Junjie and Chintala, Soumith},
booktitle = {Advances in Neural Information Processing Systems 32},
pages = {8026--8037},
year = {2019},
publisher = {Curran Associates, Inc.},
}




@misc{tvm-autotune,
  author={Wang, Yao and Yan, Eddie},
  title = {Auto-tuning a convolutional network for x86 CPU},
  howpublished = {\url{https://tvm.apache.org/docs/tutorials/autotvm/tune_relay_x86.html}},
  note = {Accessed: 2020-09-30},
  year = {2019}
}

@article{Sioutas20,
author = {Sioutas, Savvas and Stuijk, Sander and Basten, Twan and Corporaal, Henk and Somers, Lou},
title = {Schedule Synthesis for Halide Pipelines on GPUs},
year = {2020},
issue_date = {August 2020},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {17},
number = {3},
issn = {1544-3566},
url = {https://doi.org/10.1145/3406117},
doi = {10.1145/3406117},
journal = {ACM Trans. Archit. Code Optim.},
month = aug,
articleno = {23},
numpages = {25},
keywords = {GPU, image processing, Loop optimizations, Halide, scheduling}
}

@inproceedings{Sioutas18,
author = {Sioutas, Savvas and Stuijk, Sander and Corporaal, Henk and Basten, Twan and Somers, Lou},
title = {Loop Transformations Leveraging Hardware Prefetching},
year = {2018},
isbn = {9781450356176},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3168823},
doi = {10.1145/3168823},
booktitle = {Proceedings of the 2018 International Symposium on Code Generation and Optimization},
pages = {254–264},
numpages = {11},
keywords = {compiler optimizations, Halide, loop optimizations},
location = {Vienna, Austria},
series = {CGO 2018}
}

@inproceedings {Ansor20,
title = {Ansor: Generating High-Performance Tensor Programs for Deep Learning},
author={Lianmin Zheng and Chengfan Jia and Minmin Sun and Zhao Wu and Cody Hao Yu and Ameer Haj-Ali and Yida Wang and Jun Yang and Danyang Zhuo and Koushik Sen and Joseph E. Gonzalez and Ion Stoica},
booktitle = {14th {USENIX} Symposium on Operating Systems Design and Implementation ({OSDI} 20)},
year = {2020},
address = {Banff, Alberta},
url = {https://www.usenix.org/conference/osdi20/presentation/zheng},
publisher = {{USENIX} Association},
month = nov,
}


@book{rl_intro,
  added-at = {2019-07-13T10:11:53.000+0200},
  author = {Sutton, Richard S. and Barto, Andrew G.},
  biburl = {https://www.bibsonomy.org/bibtex/2f46601cf8b13d39d1378af0d79438b12/lanteunis},
  edition = {Second},
  interhash = {ac6b144aaec1819919a2fba9f705c852},
  intrahash = {f46601cf8b13d39d1378af0d79438b12},
  keywords = {},
  publisher = {The MIT Press},
  timestamp = {2019-07-13T10:11:53.000+0200},
  title = {Reinforcement Learning: An Introduction},
  url = {http://incompleteideas.net/book/the-book-2nd.html},
  year = {2018 }
}


@inproceedings{flextensor,
  author = {Zheng, Size and Liang, Yun and Wang, Shuo and Chen, Renze and Sheng, Kaiwen},
  title = {FlexTensor: An Automatic Schedule Exploration and Optimization Framework for Tensor Computation on Heterogeneous System},
  year = {2020},
  isbn = {9781450371025},
  publisher = {Association for Computing Machinery},
  address = {New York, NY, USA},
  url = {https://doi.org/10.1145/3373376.3378508},
  doi = {10.1145/3373376.3378508},
  pages = {859–873}, 
  numpages = {15},
  keywords = {machine learning, heterogeneous systems, compiler optimization, code generation},
  location = {Lausanne, Switzerland},
  series = {ASPLOS '20}
}

